Excitons and carriers in transient absorption and time-resolved ARPES spectroscopy: an abinitio approach

I present a fully abinitio scheme to model transient spectroscopy signals in presence of strongly bound excitons. Using LiF as a prototype material, I show that the scheme is able to capture the exciton signature both in time-resolved ARPES and transient absorption experiments. The approach is completely general and can become the reference scheme for modelling pump and probe experiment in a wide range of materials.

==> alias1.tex <==
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}

\newcommand{\Id}[1] {\int \! \! {\rm d}^3 #1}
\newcommand{\tens}[1] {\underline{\underline{ #1}}}
%\newsymbol\lessgtr 1337
\renewcommand{\v}[1]{{\bf #1}}


\def\nnpkkp {\begin{subarray}{l} n n'\\ \kk \kk' \end{subarray}}
\def\nmkp   {\begin{subarray}{l} n m\\ \kk \pp \end{subarray}}
\def\mnpk   {\begin{subarray}{l} m n\\ \pp \kk \end{subarray}}
\def\nnkk   {\begin{subarray}{l} n n\\ \kk \kk \end{subarray}}
\def\mnppkp {\begin{subarray}{l} m n'\\ \pp \kk' \end{subarray}}
\def\ai	{{\em ai}}
\def\abinitio	{{\em ab initio}}
\def\zero	{{\bf 0}}
\def\qw		{{\bf q},\omega}
\def\ql  	{{\bf q},\lambda}
\def\rw		{{\bf r},\omega}
%\def\rt		{{\bf r},t}
%\def\rtp	{{\bf r},t'}
\def\tone   {t_{1}}
\def\ttwo   {t_{2}}
\def\taoone   {\tau_{1}}
\def\taotwo   {\tau_{2}}
\def\ttmto   {\tau_{2}-\tau_{1}}
\def\tomtt   {\tau_{1}-\tau_{2}}
\def\pp		{{\bf p}}
\def\rr		{{\bf r}}
\def\rrp	{{\bf r}'}
\def\rrone	{{\bf r}_1}
\def\rrtwo	{{\bf r}_2}
\def\vv		{{\bf v}}
\def\wtwhH		{\widetilde{\widehat{H}}}
\def\wtwhW		{\widetilde{\widehat{W}}}
\def\FF		{{\bf F}}
%\def\AA		{{\bf A}}
\def\BB		{{\bf B}}
\def\GG		{{\bf G}}
\def\RRI        {{\bf R}_{Is}}
\def\RRJ        {{\bf R}_{Js'}}
\def\RR		{{\bf R}}
\def\OO		{{\bf O}}
\def\TT		{{\bf T}}
\def\RRp	{{\bf R'}}
\def\TTu	{\underline{\bf T}}
\def\RRu	{\underline{\bf R}}
\def\RRpu	{\underline{\bf R'}}
\def\brank  { \la n\kk \[\{\RR\}\]|}
\def\ketmp  { | m\pp \[\{\RR\}\]\ra}
\def\PP		{{\bf P}}
\def\KK		{{\bf K}}
\def\HH		{{\bf H}}
\def\UU		{{\bf U}}
\def\EE		{{\bf E}}
\def\qq		{{\bf q}}
\def\kk		{{\bf k}}
\def\qq		{{\bf q}}
\def\jj		{{\bf j}}
\def\calGzero   {{\cal G}^{(0)}}
\def\calG       {{\cal G}}
\def\intr	{\int\,d{\bf r}\,}
\def\intrp	{\int\,d{\bf r}'\,}
\def\introne	{\int\,d{\bf r}_{1}\,}
\def\intrtwo	{\int\,d{\bf r}_{2}\,}
\def\intao     {\int\,d\tau\,}

\def\eee         {{\bf e}}
\def\dd         {{\bf d}}
\def\ga         {\alpha}
\def\gb         {\beta}
\def\gc         {\gamma}
\def\gC         {\Gamma}
\def\gd         {\delta}
\def\gD         {\Delta}
\def\gee        {\epsilon}
\def\gl         {\lambda}
\def\gL         {\Lambda}
\def\go         {\omega}
\def\gO         {\Omega}
\def\goql       {\omega_{\qq \gl}}
\def\gql        {\qq \gl}
\def\gon        {\omega_{n}}
\def\goj        {\omega_{j}}
\def\goi        {\omega_{i}}
\def\igon       {i\omega_{n}}
\def\igoi       {i\omega_{i}}
\def\igoj       {i\omega_{j}}
\def\gr         {\rho}
\def\gs         {\sigma}
\def\gS         {\Sigma}
\def\gSnko      {\Sigma_{\nk}(\go)}
\def\Skon       {\Sigma(\kk,\gon)}
\def\Snko       {\Sigma_{n\kk}(\go)}
\def\Snkoi      {\Sigma_{n\kk}(\goi)}
\def\gt         {\theta}
\def\gu         {\tau}
\def\gup         {\tau'}
\def\ek         {\gee_{\bf k}}
\def\ekpq       {\gee_{\bf {k+q}}}
\def\ep         {\gee_{p}}
\def\capo       {\right.\\ \left.}
\def\dn         {\downarrow}
\def\up         {\uparrow}
\def\rar        {\rightarrow}  
\def\la         {\langle}
\def\ra         {\rangle}
\def\dg         {\dagger}
\def\grG        {\gr_{nn'}(\kk,\qq,{\bf G})}
\def\grGo       {\gr_{nn'}(\kk,\qq,{\bf G_1})}
\def\grGts      {\gr_{nn'}^*(\kk,\qq,{\bf G_2})}
\def\uob        {\frac {1}{\gb}}
\def\uoZ        {\frac {1}{Z}}
\def\uot        {\frac {1}{2}}
\def\uop        {\frac {1}{\pi}}
\def\uon        {\frac {1}{N_{\qq}}}
\def\sumon      {\sum_{n=-\infty}^{+\infty}}
\def\sumoj      {\sum_{j=-\infty}^{+\infty}}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\def\aapp       {{\em  adiabatic approximation}}
\def\MBPT       {many-body perturbation theory}
\def\MB         {many-body }
\def\GS         {ground state }
\def\GF         {Green's function }
\def\GFv        {Green's function, }
\def\GFs         {Green's functions }
\def\zpme         {zero point motion effect}

\def\nk         {n{\bf k}}
\def\nku        {n_1{\bf k}_1}
\def\nkp        {n'{\bf k}'}
\def\npp        {n'{\bf p}}
\def\nukmq      {n_1\({\bf k-q}\)}
\def\npkmq      {n'\({\bf k-q}\)}
\def\dk         {\frac{d\,{\bf k}}{\(2 \pi\)^3}}
\def\dk1        {\frac{d\,{\bf k}_1}{\(2 \pi\)^3}}
\def\dq         {\frac{d\,{\bf q}}{\(2 \pi\)^3}}

\def\dk         {\frac{d\,{\bf k}}{\(2 \pi\)^3}}
\def\dku        {\frac{d\,{\bf k}_1}{\(2 \pi\)^3}}
\def\dq         {\frac{d\,{\bf q}}{\(2 \pi\)^3}}

%%% Aliases for Chapter 2 %%%
\def\ecut       {\it E_{cut} }
\def\tpa        {{\it trans}-polyacetylene}
\def\Tpa        {{\it Trans}-polyacetylene}
\def\tpe        {polyethylene}

%%% More aliases for Chapter 2-3 %%%
\def\Hscf       {H_{scf} }
\def\Vscf       {\hat{V}_{scf} }
\def\Vxc        {\hat{V}_{xc} }

%%% Aliases for Chapter 3 %%%
\def\epc        {electron-phonon coupling }
\def\epcp        {electron-phonon coupling. }
\def\epcv        {electron-phonon coupling, }
\def\epi        {electron-phonon interaction }
\def\epip        {electron-phonon interaction.}
\def\epiv        {electron-phonon interaction,}
\def\ep         {electron-phonon }
\def\dw         {Debye-Waller }
\def\se         {self-energy }
\def\Se         {Self-energy }
\def\sep         {self-energy. }
\def\sev         {self-energy, }

\def\nk         {n{\bf k}}
\def\npkp       {n' \kk'}
\def\npk        {n' \kk}
\def\rnpk       {\mid  n'    \kk    \ra}
\def\lnpk       {\la   n'    \kk    \mid}
\def\rnk        {\mid  n     \kk    \ra}
\def\lnk        {\la   n     \kk    \mid}
\def\rnpkp      {\mid  n'    \kk'   \ra}
\def\lnpkp      {\la   n'    \kk'   \mid}
\def\rnpkpq     {\mid  n',{\bf k+q} \ra}
\def\npkmq      {n' {\bf k-q}}
\def\npkpq      {n' {\bf k+q}}

\def\uu		{{\bf u}_{Is}}
\def\uais	{u_{\ga,Is}}
\def\ubis	{u_{\gb,Is}}
\def\ubjsp	{u_{\gb,Js'}}

%%% bar %%%
\def\nt {\bar{n}}
\def\mt {\bar{m}}
%\def\itt{\bar{i}}
\def\jt {\bar{j}}
\def\wt {\bar{\omega}}
\def\blxt {\bar{\mathbf{x}}}
\def\st {\bar{\s}}

%%% Aliases for Chapter 4 %%%
\def\tlim        {T going to zero limit}
\def\bql         {\hat{b}_{\qq \gl}}
\def\bmql        {b_{-\qq \gl}}
\def\bdql        {\hat{b}^{\dg}_{-\qq \gl}}
\def\bdpql       {\hat{b}^{\dg}_{\qq \gl}}
\def\gsq         {{\mid g^{\gql}_{n' n \kk} \mid}^2}
\def\Sf          {spectral function}
\def\Sfs         {spectral functions}
\def\qp          {quasiparticle}

%%% Aliases for Journals %%%
\def\prl         {Phys. Rev. Lett. }
\def\prb         {Phys. Rev. B }
\def\pr          {Phys. Rev. }
\def\rpm         {Rev. Mod. Phys. }
\def\jpc         {J. Phys. Chem. }
\def\jp          {J. Phys. C }
\def\jcp         {J. Chem. Phys. }
\def\pss         {Phys. Stat. Sol. }

%%% More aliases for Appendix %%%
\def\self       {\epsfig{figure=Appendix/logo.ps,height=.5cm}\,}
\def\bverb      {\renewcommand{\baselinestretch}{1}\begin{verbatim}}
\def\everb  	{\end{verbatim}\renewcommand{\baselinestretch}{1.3}}


\newcommand{\yambo} {{\normalfont\ttfamily yambo\ }}


